Backpropagated Neighborhood Aggregation for Accurate Training of Spiking Neural Networks

While backpropagation (BP) has been applied to spiking neural networks (SNNs) achieving encouraging results, a key challenge involved is to backpropagate a continuous-valued loss over layers of spiking neurons exhibiting discontinuous all-or-none firing activities. Existing methods deal with this difficulty by introducing compromises that come with their own limitations, leading to potential performance degradation. We propose a novel BP-like method, called neighborhood aggregation (NA), which computes accurate error gradients guiding weight updates that may lead to discontinuous modifications of firing activities. NA achieves this goal by aggregating finite differences of the loss over multiple perturbed membrane potential waveforms in the neighborhood of the present membrane potential of each neuron while utilizing a new membrane potential distance function. Our experiments show that the proposed NA algorithm delivers the state-of-the-art performance for SNN training on several datasets.

==> feedback.tex <==

\setlength{\columnsep}{0.2cm}
\begin{wrapfigure}{r}{6cm}
    \vspace{-0.3cm}
    \centering
    \includegraphics[width=0.35\textwidth]{rebuttal.pdf}
    \label{fig:1}
    \vspace{-1cm}
\end{wrapfigure}
\setcounter{figure}{0}
\setcounter{equation}{0}

\section{Author feedback}

We deeply appreciate all the insightful review comments.

\textbf{Writing quality and citations:} We will fix all writing glitches, improve clarity and quality of writing, correct the confusions, and cite the missing references in our final paper with the major issues responded below:

\textbf{Clarification of neighbors selection (Review (R) \#5, \#7):}
We used the simple neighborhood selection (SNS) method as described in Section 3.2 in experiment. 
Fig.A is a neuron's current membrane potential $\boldsymbol{u}$ and its output spike train $\boldsymbol{s}$. We flip the firing status of the $p^{th}$ time-step to get the $p^{th}$ neighbor $\boldsymbol{u}_p$. Due to the chain-effect, the final waveform $\boldsymbol{u}_p'$ differs from $\boldsymbol{u}$ on all $t>p$ ($\rightarrow$Fig.B).

As \textbf{R \#5} suggests, one can change the size of neighborhood, yet how to find the most important several neighbors remains as future work. Based on the fact that the nearest neighbors shall differ from the present spike train on at least one time step, we take a first approach - SNS, to solve this problem. Our distance measure MP-dist may inspire future works to come up with better neighbors selection methods as discussed later. Different neighbors selection methods also lead to a varying time complexity:

\textbf{Time complexity analysis (R \#3, \#5):}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.42\textwidth]{Time.pdf}
%     \vspace{-0.4cm}
%     \caption{Wall-clock time (MNIST, TITAN XP, batch size=64)}
%     \label{fig:time}
%     \vspace{-0.7cm}
% \end{figure}
(Fig.C: MNIST, TITAN XP, BatchSize=64): NA is faster than TSSL-BP when $N_t=5$. The time complexity of both STBP and TSSL-BP is $\mathcal{O}(N_t)$. NA's time complexity is $\mathcal{O}(N_t^2)$. NA considers $N_t$ neighbors ($\rightarrow N_t$), and calculates the chain-effect forward process for each of them ($\rightarrow N_t^2$).  Future works may lower the time complexity by choosing fewer but more important neighbors (as interestingly suggested by \textbf{R \#5}).

\textbf{Distance-measure (MP-dist) quality (R \#3, \#5, \#7)}
MP-dist is not a true distance measure \textbf{(R \#7)} in a rigorous mathematical sense, and only designed for NA. The finite difference calculated by ($\Delta ~loss/\Delta~\boldsymbol{u}$) required in NA highly relies on an accurate measure of $\Delta~\boldsymbol{u}$ between the current $\boldsymbol{u}$ and its neighbor $\boldsymbol{u}_p'$: while inducing discrete jumps in firing activity, small weight updates in training shall modify the present $\boldsymbol{u}$ to a close neighbor $\boldsymbol{u}_p'$ that corresponds to a small MP-dist from $\boldsymbol{u}$.   
%Although $\boldsymbol{u}$ has jumping changes to $\boldsymbol{u}_p'$ when spike train pattern change, a good distance measure should keep small between $\boldsymbol{u}$ and $\boldsymbol{u}_p'$ under the steady training process using gradient-descent.

We evaluated the quality of MP-dist in  a practical training setting w/ a small learning rate in the experiment in \textbf{Sec. 4.2}. We tracked all possible discrete spike train pattern changes for all neurons caused by training, and computed the MP-dist for each pair of the spike trains (before \& after a weight update).The results confirmed the quality of MP-dist: a large majority of the neurons indeed change to a new spike train with a small MP-dist.   
%We rank all possible discrete spike trains under MP-dist for all neurons, and count how many changes falls into the top-k most close spike trains. The results successfully conformed the design of MP-dist: most of the neurons only change its status to their neighbors with the smallest norm of MP-dist.

\textbf{Relation to activation \& timing-based methods (R \#3, \#4, \#7)}
SNN training relies on accurate adjusting of each neuron's discontinuous all-or-none firing activity. Previous activation-based surrogate gradient methods adjust neurons' firing activity by smoothing the  activation function for all neurons prior to training,
%through macro-level averaging of loss landscapes, 
which blurs  spike timing. Differently, our NA algorithm individually analyzes each neuron at every step of training: we compute the \emph{dependency of the loss around the present membrane potential waveform $\bm u$ of each  neuron} within its neighborhood $\bm N_u$ (corresponding to discretely different spike trains) by aggregating the \emph{finite differences} of the loss between each member of $\bm N_u$ and $\bm u$. $\bm N_u$ captures close discrete changes of spike trains, which may be resulted from  addition, removal of spikes, and fine timing shifts. Hence, we claim that NA handles adding/removing and timing shifts of spikes better than previous methods, which may have contributed to the observed performance improvements in our experiments \textbf{(R \#7)}.
%NA calculates true finite difference between the current status and its nearby neighbors. The adjusting direction is well understood based on the loss change between different firing status. The choose of neighbors include changes induced by both adding/removing and timing shifts naturally. Moreover, we noticed the performance lift on several main stream datasets, so we claim NA handles both adding/removing and timing shifts of spikes better than previous methods \textbf{(R \#7)}.

\textbf{Relation to BPTT and (Kim et al., 2020) (R \#4)}
Indeed, this work was motivated deeply by the issues brought up in (Kim et al., 2020) and BPTT.  But we ended up with a totally different method. (Kim et al., 2020)  averages the gradients of activation-based and timing-based methods. Strictly speaking, NA is not a gradient-based method; it captures the discrete nature of spike train changes using the neighborhood, MP-dist, and an efficient pipeline. Please see the last comment as well.  
%NA comes with several important new concepts: neighborhood, MP-dist, and a computation efficient gradient aggregation pipeline. Compared to BPTT, the NA gradient is not \textbf{\emph{back}}-propagated within a layer from error $\boldsymbol{e}$ to $\boldsymbol{u}$, but relies on a \textbf{\emph{forward}} process $\mathscr{F}(\cdot)$ to calculate an aggregated finite difference instead.

% \begin{figure}[t]
%     \vspace{-0.1cm}
%     \centering
%     \includegraphics[width=0.45\textwidth]{rebuttal.pdf}
%     \label{fig:na}
%     \vspace{-0.7cm}
% \end{figure}

\textbf{Related works (R \#3):} We briefly comment on the related works below and will discuss more in our revised paper.(Huh and Sejnowsi, 2018) presents a BP method for recurrent SNNs based on the combination of a gate function and threshold-triggered synaptic model that is introduced to handle the non-differentiability of spikes. 
% It formulates the BP process via the continuous postsynaptic without directly involving spike timing and spike timing is one of the goals in our work. Moreover, t
The depolarization of membrane potential within a narrow active zone below the firing threshold induces a graded postsynaptic current.  Differently, we directly consider the all-or-none characteristics of firing spikes. (Bellec et al., 2018) proposes a new type of SNNs, named LSNNs, with adapting neurons and support for learning to learn. In our work, we focus on more accurate weight updates in lieu of the discrete nature of spiking activity changes, which is one of the fundamental problems of BP training.

\begin{small}
Kim,  J.,  Kim,  K.,  and  Kim,  J.-J. Unifying  activation-and timing-based learning rules for Spiking Neural Networks. \emph{NeurIPS.} 2020.

Huh, Dongsung, and Terrence J. Sejnowski. "Gradient descent for spiking neural networks." \emph{NeurIPS.} 2018.

Bellec, Guillaume, et al. "Long short-term memory and learning-to-learn in networks of spiking neurons." \emph{NeurIPS.} 2018.
\end{small}

==> methods.tex <==
\section{Methods}
% \label{sec:methods}
% To apply BP algorithm on the SNNs' optimization problem, we need to firstly understand what are the neighbor points of a neuron's PSC.
% \subsection{neuron PSC's Neighborhood}
% As mentioned above, all possible PSC patterns of a neuron only occupy a small subset $\mathds{P} \subset \mathds{R}_T$, where $T$ is the number of discrete time-steps. To define the neighborhood of a PSC point $p\in\mathds{P}$, we need to firstly define the distance between two patterns. Since the neuron's PSC $a$ has its sole corresponding spike-trains $S$, and both of them are decided by the neuron's membrane potential $U$, we can consider the distance using these three variables together. Here we provide three versions of distance definition.
% \subsubsection{Discrete spike distance}
% \begin{figure*}[t]
%     \centering
%     % \vspace{-0.2cm}
%     \includegraphics[width=\textwidth]{distance_v1.pdf}
%     \vspace{-0.6cm}
%     \caption{Discrete Spike Distance experiment results}
%     \label{fig:distance_v1}
% % \vspace{-0.6cm}
% \end{figure*}

% If only take the spike-trains $S$ into consideration, we can get a relatively simple yet effective distance metric. Following the same idea like Hamming distance \cite{hamming1950error} / Damerau-Levenshtein Distance \cite{damerau1964technique}, the "Discrete Spikes Distance" between two binary strings with equal length is now defined as the following:\par
% \theoremstyle{definition}
% \begin{definition}[Discrete Spikes Distance]
% 1. The distance measures the minimum number of "moves" required to transform one string into the other.
% 2. The moves include:
% ~~1) Flip (spikes generate | vanish)
% ~~2) Swap (spikes move)
% \end{definition}
% The changes of the patterns under the new definition would have their sole corresponding interpretations. Figure \ref{fig:distance_v1} (a) shows the distance between different spike-trains under the above distance definition. Closer spike-trains are represent by lighter color. If we sorted the spike-trains line by line, we could get Figure \ref{fig:distance_v1} (b). Using it as the background to visualize the relationship between the distance metric and experiment spike-trains transformation frequency, in Figure \ref{fig:distance_v1} (c), we plot the transfer matrix again, but using distance sorted (order-preserving) spike-trains as x-axis, where we can see most neurons output transfer between two spike-trains with small distance. In Figure \ref{fig:distance_v1} (d), we sum up all spike-trains to stat the overall relationship between number of transformation / accumulated probability with the discrete spike distance. 61\% of transformations happens within top 10 closest points among all 1024 points.\par We provide a pseudo-code as shown below:\par
% \begin{algorithm}[h]
%     \SetAlgoLined
%     \textbf{Input} $\overrightarrow{spikeTrain_I},\overrightarrow{spikeTrain_N}$; \\
%     \textbf{Output} $Dist$; \\
%     initialization $S_I'=S_N'=\textbf{Null}$, $Dist'=Dist=0$ $Paired=\textbf{False}$; \\
%     \For {$i=1,2,\ldots,T$}{
%     $S_I=\overrightarrow{spikeTrain_I}[i],~S_N=\overrightarrow{spikeTrain_N}[i]$;\\
%     \If{$S_I$ {\rm not equal to} $S_N$}{
%         \eIf{Paired ==\textbf{False} and $S_I$==$S_N'$ and $S_N$==$S_I'$}{
%             $Dist=Dist'$;\\
%             $Paired = \textbf{True}$;
%         }{
%             $Dist'=Dist$;\\
%             $Dist=Dist'+1$;\\
%             $Paired = \textbf{False}$;
%         }
%     }
%     $S_I'= S_I, S_N'=S_N$;
%     }
% \caption{Discrete spike distance}
% \label{algo:discrete}
% % \vspace{-0.05cm}
% \end{algorithm}
% \vspace{-0.15cm}
% \subsubsection{Continuous spike distance}
% \begin{figure}[h]
%     \centering
%     % \vspace{-0.2cm}
%     \includegraphics[width=0.48\textwidth]{icml_fg3.pdf}
%     \vspace{-0.6cm}
%     \caption{Discrete / Continuous Spike Distance example}
%     \label{fig:distance_v1&v2}
% \vspace{-0.4cm}
% \end{figure}
% Take both of membrane potential $U$ and spike-trains $S$ into consideration. For the flip operation, when a neuron's $U$ near the threshold $\vartheta$, its output will be more easily to flip. Moreover, we wish to keep the range of distance of one move $\in[0,1]$ So the distance on that time-step is defined as $min(1,|(U-\vartheta)|)$. As for swap operation, since the $U$ on two near time-steps need to cross the threshold at the same time, and to maintain the range of distance, the distance of swap operation is defined as $\frac{1}{2}\cdot(min(1,|(U_1-\vartheta)|)+min(1,|(U_2-\vartheta)|))$. Figure~\ref{fig:distance_v1&v2} shows the first two metrics' difference. By adding membrane potential's information, the original distance 3 is reduced to 0.55 under the new metric. The pseudo-code of the Continuous spike distance is shown in the Algorithm \ref{algo:continuous}.

% \begin{algorithm}[h]
%     \SetAlgoLined
%     \textbf{Input} $\overrightarrow{spikeTrain_I},\overrightarrow{spikeTrain_N},$ $\vec{U}$; \\
%     \textbf{Output} $Dist$; \\
%     initialization $S_I'=S_N'=\textbf{Null}$,$Dist'=Dist=0$, \\ $~~~~~~~~~Paired=\textbf{False}$; \\
%     \For {$i=1,2,\ldots,T$}{
%     $S_I=\overrightarrow{spikeTrain_I}[i],~S_N=\overrightarrow{spikeTrain_N}[i]$;\\
%     \If{$S_I$ {\rm not equal to} $S_N$}{
%         \eIf{Paired ==\textbf{False} and $S_I$==$S_N'$ and $S_N$==$S_I'$}{
%             $Dist=Dist'+\frac{1}{2}\cdot(min(1,|(\vec{U}[i-1]-\vartheta)|)$\\
%             $~~~~~~~~~~+min(1,|(\vec{U}[i]-\vartheta)|))$;\\
%             $Paired = \textbf{True}$;
%         }{
%             $Dist'=Dist$;\\
%             $Dist=Dist+min(1, |\vec{U}[i]-\vartheta|)$;\\
%             $Paired = \textbf{False}$;
%         }
%     }
%     $S_I'= S_I, S_N'=S_N$;
%     }
% \caption{Continuous spike distance}
% \label{algo:continuous}
% % \vspace{-0.05cm}
% \end{algorithm}
% \vspace{-0.15cm}
% \subsubsection{Chain effect spike distance}
% To capture the complex timing dynamics of a neuron, we consider the temporal dependency between time-steps into the distance metric. If the membrane potential $U$ on the time-step $t$ jump over the threshold $\vartheta$, the neuron would fire a spike, and reset membrane potential to zero, so the next time-step's $U[t+1]$ would inherit nothing from $U[t]$. So if the $S[t+1]$ originally fires, and membrane potential $U[t+1]$ originally not large enough ($U[t+1] < \vartheta + \left(1-\frac{1}{\tau_m}\right) * U[t]_{origin}$), the neuron's $U[t+1]$ would most likely drop down the threshold $\vartheta$, and would not fire then. The dropping down without membrane potential resetting would then rise up $U[t+2]$, and if $U[t+2]$ originally not small enough ($U[t+2] > \vartheta - \left(1-\frac{1}{\tau_m}\right) * U[t+1]_{new}$), the newly inherited membrane potential $\approx\left(1-\frac{1}{\tau_m}\right) * U[t+1]_{new}$ might flip $S[t+2]$ to fire, and so on. Such step by step influence is named as Spike-trains' \textbf{Chain Effect}.The pseudo-code is shown in the algorithm \ref{algo:chain}.

% \begin{algorithm}[h]
% \SetAlgoLined
%     \textbf{Input} $\overrightarrow{spikeTrain_I},\overrightarrow{spikeTrain_N}, \vec{U}$; \\
%     \textbf{Output} $Dist$; \\
%     initialization $S_I'=S_N'=\textbf{Null}$, $Dist'=Dist=0$, \\  $~~~~~~~~~Paired=\textbf{False}$, $U'=U''=0$; \\
%     \For {$i=1,2,\ldots,T$}{
%     $S_I=\overrightarrow{spikeTrain_I}[i],~S_N=\overrightarrow{spikeTrain_N}[i]$;\\
%     $spike=(\vec{U}[i]-\vartheta)>0$;\\
%     \If{$int(spike)$ {\rm not equal to} $S_I$}{
%         $S_I = 1-S_I$;\\
%         $U'=\vec{U}[i+1]$;\\
%         $\vec{U}[i+1]$+=
%         \begin{math}
%         \begin{cases}
%             -\textit{U''}\cdot (1-\frac{1}{\tau_m}),~ spike {\rm ~~is~~} \textbf{True} \\
%             \textit{U[i]}\cdot (1-\frac{1}{\tau_m}),~ spike {\rm ~~is~~} \textbf{False}
%         \end{cases}
%         \end{math};\\
%         $U''=U'$;
%     }
%     \If{$S_I$ {\rm not equal to} $S_N$}{
%         \eIf{Paired ==\textbf{False} and $S_I$==$S_N'$ and $S_N$==$S_I'$}{
%             $Dist=Dist'+\frac{1}{2}\cdot(min(1,|(U_1-\vartheta)|)\\
%             ~~~~~~~~~~+min(1,|(U_2-\vartheta)|))$;\\
%             $Paired = \textbf{True}$;
%         }{
%             $Dist'=Dist$;\\
%             $Dist=Dist+min(1, |U[i]-\vartheta|)$;\\
%             $Paired = \textbf{False}$;
%         }
%     }
%     $S_I'= S_I, S_N'=S_N$;
%     }
% \caption{Chain effect spike distance}
% \label{algo:chain}
% % \vspace{-0.05cm}
% \end{algorithm}
% \vspace{-0.15cm}
% This metric also has a simplified version. Since the membrane potential $U$ is usually near the threshold $\vartheta$ when it is about to trigger a change, we can substitute the variable $U'$ and $U''$ by the fix threshold $\vartheta$. We name this as Simple chain effect spike distance.
% \begin{figure}[b]
%     \centering
%     % \vspace{-0.2cm}
%     \includegraphics[width=0.35\textwidth]{Compare.pdf}
%     \vspace{-0.2cm}
%     \caption{The quality comparison of the three distance metrics}
%     \label{fig:compare}
% \vspace{-0.3cm}
% \end{figure}

% \subsubsection{Neighborhood Comparison}
% We compared the three distance metrics' accumulated probability in Figure \ref{fig:compare}. The chain effect spike distance is the best among all three metrics. It's top 1 near neighbor has \~63\% predict accuracy, and it's simplified version also has very close performance. The continuous / discrete spike distance need Top 4 / Top 10 near neighbors respectively to reach the comparable predict accuracy.\par
% If we made a valid \textbf{assumption}:
% Assume the learning rate is small enough during training, so that no two time-steps’ membrane potential cross the threshold together.
% Then the spike-trains can only move according to timing chain-effect. Therefore, we use chain-effect to define a spiking neuron's output's near neighborhood when applying BP algorithm.

% \subsection{Neighbor forecasting back-propagation (NFBP)}
% The BP algorithm needs to propagate the error signal $({\partial Loss}/{\partial a})$ through layers. Figure \ref{fig:path} shows the data flow of a layer according to equation (\ref{eq:1}), (\ref{eq:2}), and(\ref{eq:3}).
% The NFBP algorithm solves the calculation of $({\partial Loss}/{\partial U})$ from $({\partial Loss}/{\partial a})$ as shown in the red color.
% The arrow between $a$ and $U$ is bidirectional. Some lines are dashed. We will explain the meaning of these later.\par
% \begin{figure}[ht]
%     \centering
%     % \vspace{-0.2cm}
%     \includegraphics[width=0.48\textwidth]{path.pdf}
%     \vspace{-0.6cm}
%     \caption{Data flow path}
%     \label{fig:path}
% \vspace{-0.2cm}
% \end{figure}
% \begin{figure*}[t]
%     \centering
%     % \vspace{-0.2cm}
%     \includegraphics[width=\textwidth]{NFBP.pdf}
%     \vspace{-0.6cm}
%     \caption{The Neighbor Forecasting Back-propagation (NFBP) algorithm}
%     \label{fig:NFBP}
% % \vspace{-0.6cm}
% \end{figure*}
% % \begin{figure}[h]
% %     \centering
% %     % \vspace{-0.2cm}
% %     \includegraphics[width=0.48\textwidth]{neighbors.pdf}
% %     % \vspace{-0.6cm}
% %     \caption{Neighbors example}
% %     \label{fig:neighbors}
% % % \vspace{-0.6cm}
% % \end{figure}
% As discussed above, SNNs' training problem is a discrete space optimization problem. The continuous derivative shall be converted to finite differences between near neighbors. Our training algorithm also follows this way, and has three steps:1. Neighbors forecasting. 2.Error projection. 3. distance based differences aggregation.


% \subsubsection{Neighbors forecasting}
% The number of neighbors is equal to the number of time-steps $T$. We assume that at most one time-step's membrane potential $U$ can cross the threshold during one iteration's training when learning-rate is small. A neuron's output pattern then has totally $T$ possible neighbor-patterns. Each pattern is generated by flipping the corresponding time-step's spike-train status, and the following time-steps are determined by spike chain-effect. \par


% % Figure \ref{fig:neighbors} is a real case we got during training a SNN on the MNIST dataset. One neuron has the output spike-train $S$ as shown on the top of the Figure \ref{fig:neighbors}. The yellow colored box means the output is one on that time-step, and the dark blue colored box means no spike fires. Our neighbors forecasting algorithm provides $T$ neighbor spike-trains as shown line by line below the initial spike-train. We define the $i^{th}$ neighbor as flipping the neuron's output on the $i^{th}$ time-step, with the predicting on how the following output would change accordingly. We define these $T$ neighbors as the ten neighbor spike-trains it can transfer to.\par
% We set $T=5$ in Figure~\ref{fig:NFBP} (a), and (b) to demonstrate the \textbf{step.1} of the NFBP algorithm. In order to get the present spike-train $S$'s neighbor $S_i, i=1,2\dotsb,T$, we force a flip on the $i^{th}$ time-step of $S$ (shown by red colored boxes). Then the following spike-trains would change following the chain-effect (shown by green colored boxes. The dashed box means the output on the following time-step remains unchanged, and solid boxes means changed). The information of membrane potential $U$ does not shown in the Figure for simplification. As shown in Figure~\ref{fig:NFBP} (b), the $T$ neighbor spike-trains also has their corresponding PSCs $a_i, i=1,2\dotsb,T$, which is used to compare with the present PSC $a$ in the next step - Error projection.
% \subsubsection{Error projection}
% The back propagated $error$ signal $({\partial Loss}/{\partial a})$ implies how the neuron's output PSC $a$ diverges from the expected value. So the projection of the $-error$ signal onto the PSC changes $\Delta a_i = a_i-a$ indicates how good is the $i^{th}$ neighbor. Figure \ref{fig:NFBP} (c) shows the relationship between the error-signal and the PSC neighborhood. The more positive the projection $p_i$ is, the better to flip the spike-train $S$ on its $i^{th}$ time-step. We consider the projection $\vec{P}=[p_0, p_1,\cdot,p_T]$ as a gradient-liked indicator, but it cannot be used as gradient without step.3 - distance based differences aggregation.
% \subsubsection{Distance based differences aggregation}
% The projection $\vec{P}=[p_0, p_1,\cdot,p_T]$ indicates the wish to flip the status of a time-step's output. However, the difficulty to flip them is different. Each neighbor has different distance between itself and the current status. We measure the distance under the chain effect spike distance. Since the neighbors are also defined by the chain effect, the distance of the $i^{th}$ neighbor is simplified as $|U[i]-\vartheta|$, where we omit the upper bound one. We use an aggregation function $Dist$ as shown in Figure \ref{fig:NFBP} (d) to balance the wishes on each time-steps. The closer neighbors are easier to flip, and they would gain larger weights on the direction to go. From the aspect of high-dimensional discrete space optimization, the estimated differential gradient is an estimation using the discrete near neighbors differences, so near neighbors are weighted more. The aggregation weight function is defined as $\lambda/((U-\vartheta)^2+\lambda)$. We also tried other functions like $\lambda/(|U-\vartheta|+\lambda)$ and different values of $\lambda$. The results show that the NFBP algorithm does not sensitive to the choose of the aggregation function. We choose the first form, with $\lambda=0.2$. \par
% The term circled by the dashed purple line defines the direction to flip. The projection $P$ only encodes the wish to flip, but no direction specified. We decrease the membrane potential $U$ on a fired time-step ($S=1$, $(S-0.5)*2=1$) to extinguish it (positive gradient will decrease the value), and increase $U$ on a non-fired time-step ($S=0$, $(S-0.5)*2=-1$) to light it on (Negative gradient will increase the value).
% \subsubsection{NFBP conclusion}
% NFBP is not a typical BP-liked algorithm for two reasons. First, the gradient is not calculated by any direct approximation/randomness, but by a projection, an evaluation of how good it is to go along a dimension, with the scale proportional to the error signal to ensure convergence. Second, it is not totally calculated backward. The \textbf{step1} calculated the neighbors forward a little bit, then use the comparison to determine the underlying membrane potential's gradient (where we use bidirectional arrows in Figure \ref{fig:path} to show this).\par
% NFBP provides a better gradient takes both spatial and temporal effects into consideration. The temporal effect is back-propagated indirectly through SNNs' forward chain effect (where we use dashed lines in Figure \ref{fig:path} to show this). The chain effect determines whether the impact on the future steps PSC align with the error signal's expectation. In this way, the missing dependency between time-steps are well concluded.

% % As shown in the Figure \ref{fig:NFBP} (a), in the \textbf{step.1}, we got the neighbor spike-trains $S_i, i=1,2\dotsb,T$. The spike-trains corresponding PSCs $a_i, i=1,2\dotsb,T$ are also the neighbors of the neuron's output PSC. 

% %Then for a PSC point $p\in\mathds{P}$, we define its neighborhood $\mathds{N} \subset \mathds{P}$ as the following:
% % for any PSC pattern $p'$, 

% \subsection{Complexity analyses}
% We can make a trade off between the NFBP's space-complexity and its time-complexity. Since each neighbors computation is dependent, the NFBP algorithm can run highly parallel as shown in Figure \ref{fig:NFBP} (a). We compute all neighbors simultaneously and get the gradient on all time-steps at the same time. The space-complexity is $O(T)$. This scenario fits small size SNNs with small time-steps $T$ running on small datasets like MNIST or Fashion-MNIST very well. Whereas on larger tasks, like running on the CIFAR10 dataset with larger SNNs, or running on the N-MNIST dataset with larger time-steps $T$, the space-complexity proportional to the number of neighbors $T$ is a problem. We can instead compute each neighbors one by one, and get the gradient on each time-steps one by one. In this way, the space overhead is $O(1)$, but the time-complexity is increased from $O(T)$ to $O(T^2)$. The $T$ newly added is the number of neighbors, and the original $T$ is the chain-effect required step by step neighbors forecasting. Fortunately, the better gradient generated by NFBP enabled the training of fast-inference SNNs with small time-steps, and the chain-effect step by step neighbor forecasting usually ends much earlier than the total time-steps $T$. So we did not experience a lot reduction of training speed. We will also report our training time in the following section.
% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:
